Graph Enabled Cross-Domain Knowledge Transfer

To leverage machine learning in any decision-making process, one must convert the given knowledge (for example, natural language, unstructured text) into representation vectors that can be understood and processed by machine learning model in their compatible language and data format. The frequently encountered difficulty is, however, the given knowledge is not rich or reliable enough in the first place. In such cases, one seeks to fuse side information from a separate domain to mitigate the gap between good representation learning and the scarce knowledge in the domain of interest. This approach is named Cross-Domain Knowledge Transfer. It is crucial to study the problem because of the commonality of scarce knowledge in many scenarios, from online healthcare platform analyses to financial market risk quantification, leaving an obstacle in front of us benefiting from automated decision making. From the machine learning perspective, the paradigm of semi-supervised learning takes advantage of large amount of data without ground truth and achieves impressive learning performance improvement. It is adopted in this dissertation for cross-domain knowledge transfer. (to be continued)

==> table.tex <==
\renewcommand{\baselinestretch}{0.8}
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp} 
\let\PBS=\PreserveBackslash
\begin{table}[htbp]
\centering
\begin{minipage}{0.89\textwidth}
\caption[Major Differences Between Neural Networks and Cell Signaling Networks]{Major Differences Between Neural Networks and Cell Signaling Networks\protect\footnote{You can also have footnote in table as in figure.}}
\vskip .25in
\label{table:NN_DIFF}

  \footnotesize
    \begin{tabular}
	{|p{0.04 \textwidth}
	|p{0.15 \textwidth}
	|p{ 0.35 \textwidth}
	|p{ 0.35 \textwidth}|} \hline
	\rule{0pt}{1pt} & & & \\
	\strut & 
		\PBS\raggedright{\em Salient features of networks} &
		\PBS\raggedright{\em Neural Networks} &
		\PBS \raggedright{\em Cell Signaling Networks}\\
	\rule{0pt}{1pt}& & & \\ \hline
	\rule{0pt}{1pt}& & & \\
	\strut (i)  & 
		\PBS\raggedright{nodes} & 
		\PBS\raggedright{all nodes typically identical} &
		\PBS\raggedright{nodes are not all equivalent in performance} \\
	\rule{0pt}{1pt}& & & \\ \hline
	\rule{0pt}{1pt}& & & \\
	\strut (ii) & 
		\PBS\raggedright{structure} &
		\PBS\raggedright{typically layered with feed-forward connections only} &
		\PBS\raggedright{regulatory signals often give rise to feedback connections resulting in cycles} \\
	\rule{0pt}{1pt}& & & \\ \hline
	\rule{0pt}{1pt}& & & \\
	\strut (iii) & 
		\PBS\raggedright{connectivity} & 
		\PBS\raggedright{highly connected} &
		\PBS\raggedright{more sparsely connected} \\
	\rule{0pt}{1pt}& & & \\ \hline
	\rule{0pt}{1pt}& & & \\
	\strut (iv) &  
		\PBS\raggedright{learning rule} &
		\PBS\raggedright{connectivity altered to perform a single function e.g.,~via a back-propagation algorithm} &
		\PBS\raggedright{cells must be able to respond to multiple stimuli effectively;changes typically occur via evolutionary processes} \\

	\rule{0pt}{1pt}& & & \\ \hline
    \end{tabular}
\\
\end{minipage}
\end{table}
\renewcommand{\baselinestretch}{1.65}

